ArtTrack: Articulated Multi-person Tracking in the Wild

In this paper we propose an approach for articulated tracking of multiple people in unconstrained videos. Our starting point is a model that resembles existing architectures for single-frame pose estimation but is substantially faster. We achieve this in two ways: (1) by simplifying and sparsifying the body-part relationship graph and leveraging recent methods for faster inference, and (2) by offloading a substantial share of computation onto a feed-forward convolutional architecture that is able to detect and associate body joints of the same person even in clutter. We use this model to generate proposals for body joint locations and formulate articulated tracking as spatio-temporal grouping of such proposals. This allows to jointly solve the association problem for all people in the scene by propagating evidence from strong detections through time and enforcing constraints that each proposal can be assigned to one person only. We report results on a public MPII Human Pose benchmark and on a new MPII Video Pose dataset of image sequences with multiple people. We demonstrate that our model achieves state-of-the-art results while using only a fraction of time and is able to leverage temporal information to improve state-of-the-art for crowded scenes.

==> table_mpii_multi_deepercut.tex <==
%\renewcommand{\tabcolsep}{0.15cm}
\tabcolsep 1.5pt
\begin{table}[tbp]
 \scriptsize
  \centering
  \begin{tabular}{@{} l c ccc ccc cc@{}}
    \toprule
    Setting& Head   & Sho  & Elb & Wri & Hip & Knee & Ank & AP & time, [s/f]\\
    \midrule
    \bufull, \labeling & 90.6  & 86.0  & 73.5  & 58.9  & \textbf{71.8}  & 64.2 & 53.2 & 71.3 & 1.48 \\
    \bufull            & 90.4  & 86.4  & \textbf{73.8}  & \textbf{60.6}  & 71.4  & \textbf{64.6} & \textbf{53.9} & \textbf{72.0} & 0.13 \\
    \busparse          & 90.7  & \textbf{86.8}  & 71.9  & 57.3  & 70.3  & 63.7 & \textbf{53.9} & 71.1 & 0.07 \\

    \midrule
    
    \tdbushort{} + \spatprop & \textbf{92.2}  & 85.9  & 72.8  & \textbf{63.4}  & \textbf{73.7}  & \textbf{66.4} & \textbf{58.9} & \textbf{73.3} & \textbf{0.01} \\ % exp 1051

%    \regfull, \labeling & 91.0  & 85.3  & 72.1  & 59.2  & 70.3  & 65.0 & 55.8 & 71.3 & 1.3 \\
%    \regfull            & 90.9  & 86.1  & 72.4  & 60.9  & 70.1  & 65.6 & 56.5 & 71.8 & 0.2 \\
%    \regsparse \\
    
    
    % final numbers after rerunning all experiments - to put in final version

    % my spatial pairwise
    % \regfull, \labeling & 91.0  & 85.3  & 72.1  & 59.2  & 70.3  & 65.0 & 55.8 & 71.3 & 0.90 \\ % exp 1108 median 0.90 mean 1.535554555
    % \regfull & 90.9  & 86.1  & 72.4  & 60.9  & 70.1  & 65.6 & 56.5 & 71.8 & 0.13 \\ % exp 1109 median 0.128679 mean 0.244549705
    % \regsparse & 90.9  & 86.5  & 68.9  & 53.8  & 68.2  & 60.9 & 51.4 & 68.7 & 0.07 \\ median 0.065648 mean 0.117189502513

    % micha spatial pairwise
    % \regfull, \labeling & 90.0  & 84.9  & 71.1  & 58.4  & 69.7  & 64.7 & 54.7 & 70.5 & 1.48 \\ % exp 1107 median 0.90 mean 1.535554555
    % \regfull            & 91.2  & 86.0  & 72.9  & 61.5  & 70.4  & 65.4 & 55.5 & 71.9 & 0.13 \\ % exp 1111 median 0.207705 mean 0.41995202
    % \regsparse          & 91.1  & 86.5  & 70.7  & 58.1  & 69.7  & 64.7 & 53.8 & 70.6 & 0.07 \\ exp 1112 median 0.065506 mean 0.130323885
    %\tdbushort{} + \spatprop & 92.2  & 86.1  & 72.8  & 63.0  & 74.0  & 66.2 & 58.4 & 73.3 & 0.01 \\ % exp 1052, 1113 median 0.011159 mean 0.013632765
    
    %\midrule
    %$\deepercut$~\cite{insafutdinov16eccv} & 78.5 & 70.5 & 59.7 & 48.7 & 55.4  & 50.6 & 44.4 & 58.7 & 270 \\
    %$\deepercut$~\cite{insafutdinov16eccv} + filter poses &  &  & &  &  &  &  &  & 270 \\
    \bottomrule
  \end{tabular}
  \vspace{0.1em}
\caption[]{Effects of various variants of $\regression$ model on pose estimation performance (AP) on MPII Multi-Person Val.}
\label{tab:mpii-single-frame-val:regression}
\end{table}


==> table_mpii_multi_person_cond_connect.tex <==
%\renewcommand{\tabcolsep}{0.15cm}
\tabcolsep 1.5pt
\begin{table}[tbp]
 \scriptsize
  \centering
  \begin{tabular}{@{} l c ccc ccc cc@{}}
    \toprule
    Setting& Head   & Sho  & Elb & Wri & Hip & Knee & Ank & UBody & FBody \\
    \midrule
    	deepercut, fully-connected \todo{} \\
        deepercut, sparse \todo{} \\
        person cond, star model \todo{}\\ 
    \bottomrule
  \end{tabular}
  \vspace{0.1em}
\caption[]{Effects of different versions of the Person Conditioned model on pose estimation (AP) on MPII Multi-Person Val}
    \vspace{-1.5em}
  \label{tab:mpii-multi-intermediate:ap}
\end{table}


==> table_mpii_multi_video.tex <==
%\renewcommand{\tabcolsep}{0.15cm}
\tabcolsep 1.5pt
\begin{table}[tbp]
 \scriptsize
  \centering
  \begin{tabular}{@{} l c ccc ccc ccc@{}}
    \toprule
    Setting& Head   & Sho  & Elb & Wri & Hip & Knee & Ank & AP \\
    \midrule
    \bufull & 84.0  & 83.8  & 73.0  & 61.3  & \textbf{74.3}  & 67.5 & 58.8 & 72.1 \\
    \quad + \temporal & 84.9  & 83.7  & 72.6  & 61.6  & \textbf{74.3}  & 68.3 & 59.8 & 72.4  \\
    \midrule
    \busparse & 84.5  & 84.0  & 71.8  & 59.5  & 74.4  & 68.1 & 59.2 & 71.9 \\
    \quad + \temporal & \textbf{85.6}  & 84.5  & 73.4  & 62.1  & 73.9  & \textbf{68.9} & \textbf{63.1} & \textbf{73.3} \\
    \midrule
    \tdbushort + \spatprop & 82.8  & 84.6  & 73.8  & 62.6  & 73.9  & 67.8 & 60.0 & 72.2 \\ % 1079
    \quad + \temporal & 83.0  & \textbf{84.8}  & \textbf{74.2}  & \textbf{63.5}  & 74.1  & 68.6 & 60.9 & 72.7 \\ % 1081
    \bottomrule
  \end{tabular}
  \vspace{0.1em}
\caption[]{Pose estimation results (AP) on our \videodata.} % \todo{Currently 28 sequences}
  \label{tab:mpii-multi-video:overall}
\end{table}

